Optimal Depth-Three Circuits for Inner Product

We show that Inner Product in $2n$ variables, $\mathbf{IP}_n(x, y) = x_1y_1 \oplus \ldots \oplus x_ny_n$, can be computed by depth-3 bottom fan-in 2 circuits of size $\mathsf{poly}(n)\cdot (9/5)^n$, matching the lower bound of G\"o\"os, Guan, and Mosnoi (Inform. Comput.'24). Our construction is obtained via the following steps. - We provide a general template for constructing optimal depth-3 circuits with bottom fan-in $k$ for an arbitrary function $f$. We do this in two steps. First, we partition $f^{-1}(1)$ into orbits of its automorphism group. Second, for each orbit, we construct one $k$-CNF that (a) accepts the largest number of inputs from that orbit and (b) rejects all inputs rejected by $f$. - We instantiate the template for $\mathbf{IP}_n$ and $k = 2$. Guided by the intuition (which we call modularity principle) that optimal 2-CNFs can be constructed by taking the conjunction of variable-disjoint copies of smaller $2$-CNFs, we use computer search to identify a small set of building block 2-CNFs over at most 4 variables. - We again use computer search to discover appropriate combinations (disjoint conjunctions) of building blocks to arrive at optimal 2-CNFs and analyze them using techniques from analytic combinatorics. We believe that the approach outlined in this paper can be applied to a wide range of functions to determine their depth-3 complexity.

==> setup/preamble.tex <==
\RequirePackage{mathtools,amsmath, amsthm, amssymb,amscd,amsfonts}
\RequirePackage{scalefnt}
\usepackage[T1]{fontenc}
\usepackage{slantsc}
\usepackage[utf8]{inputenc}
\RequirePackage[dvipsnames]{xcolor}
\usepackage{lmodern}
\usepackage{bbm}
\usepackage{comment}
\usepackage[mathscr]{euscript}
\RequirePackage[letterpaper,top=1in,bottom=1in,left=1in,right=1in]{geometry}
\RequirePackage{tikz,pgf}
\RequirePackage{graphicx}
\RequirePackage[classfont=bold,langfont=roman,funcfont=typewriter,full,classfont=bold,langfont=caps,funcfont=typewriter,full]{complexity}
\RequirePackage{algpseudocode,algorithm,algorithmicx}
\usepackage{todonotes}
\usepackage[colorlinks=true,citecolor=blue,linkcolor=blue]{hyperref}
\hypersetup{
    colorlinks,
    linkcolor={red!50!black},
    citecolor={blue!50!black},
    urlcolor={blue!80!black}
}

\usepackage[nameinlink, noabbrev, capitalize]{cleveref}
\usepackage[inline]{enumitem}

\usepackage[
backend=biber,
style=alphabetic,
sorting=nyt,
maxnames=8,
maxalphanames=8,
% sortcites,
backref=true,
url=false
]{biblatex}

\usepackage{subfiles}
% \usepackage{minted}

\AtBeginDocument{%
  \DeclareFontShape{T1}{lmr}{m}{scit}{<->ssub*lmr/m/scsl}{}%
}



%Algorithmicx package
%\algrenewcommand\algorithmicrequire{\textbf{Input:}}
%\algrenewcommand\algorithmicensure{\textbf{Output:}}
%\RequirePackage[12tabu, orthodox]{nag}
%\RequirePackage{caption}
%\RequirePackage{siunitx}
%\RequirePackage{verbatim}
%\RequirePackage{enumerate}
%\RequirePackage{fancyvrb}
%\RequirePackage{float}
%\usepackage{mathrsfs} %formal math script font
%\usepackage{bbm}
%\RequirePackage{braket}
%\usepackage{natbib}
%\usepackage{bibentry}
%\nobibliography*

